Speech Pseudonymisation Assessment Using Voice Similarity Matrices

The proliferation of speech technologies and rising privacy legislation calls for the development of privacy preservation solutions for speech applications. These are essential since speech signals convey a wealth of rich, personal and potentially sensitive information. Anonymisation, the focus of the recent VoicePrivacy initiative, is one strategy to protect speaker identity information. Pseudonymisation solutions aim not only to mask the speaker identity and preserve the linguistic content, quality and naturalness, as is the goal of anonymisation, but also to preserve voice distinctiveness. Existing metrics for the assessment of anonymisation are ill-suited and those for the assessment of pseudonymisation are completely lacking. Based upon voice similarity matrices, this paper proposes the first intuitive visualisation of pseudonymisation performance for speech signals and two novel metrics for objective assessment. They reflect the two, key pseudonymisation requirements of de-identification and voice distinctiveness.

==> intro_nick.tex <==
The proliferation of speech technologies and the increase in data protection regulation such as the European General Data Protection Regulation (GDPR) has fueled interests in privacy preservation solutions for speech data~\cite{NAUTSCH2019441}. There are two general strategies: encryption and anonymisation.  Encryption is applied to protect speech data from interception and eavesdropping.  Anonymisation, the focus in this paper, aims to ensure that speech data cannot be linked to the original speaker.

With very few solutions having been proposed, and with the few existing solutions achieving only modest levels of anonymisation, the VoicePrivacy initiative\footnote{\url{https://voiceprivacychallenge.org/}}~\cite{tomashenko2020voiceprivacy} was launched in 2019 to promote the consideration of privacy and to foster progress in privacy preservation.  VoicePrivacy 2020 takes the form of a challenge in which participants are tasked with the development of anonymisation solutions to (i)~suppress 
(as much as possible) the
speaker identity from an utterance while nonetheless preserving speaker distinctiveness and (ii)~leave intact 
(as much as possible) 
the linguistic content, quality and naturalness.
%and while preserving 
%(as much as possible) 
%voice uniqueness.
The requirement for voice uniqueness implies that anonymised voices remain distinguishable and that all utterances from the same original speaker are anonymised with the same \emph{pseudovoice}.  We hence refer to this requirement as \emph{pseudonymisation}.

While VoicePrivacy stands to make substantial inroads, 
%into privacy research for speech, 
it is clear that the metrics used to assess pseudonymisation performance are far from being straightforward; they must reflect multifaceted criteria.  The work in this paper is concerned with metrics that reflect criteria related exclusively to the speaker \emph{identity} or, more specifically, de-identification; it is not concerned with complementary metrics for assessing the preservation of linguistic content etc.  Most of the prior work including VoicePrivacy, e.g.~\cite{fang2019speaker,srivastava2019evaluating,tomashenko2020voiceprivacy}, measures privacy using trivial, generic metrics such as the equal error rate (EER) estimated from automatic speaker verification (ASV) experiments.  The general idea is to gauge performance by comparing the EER using original speech data to that obtained using speech data after de-identification ; the greater the difference, or the higher the EER, the better the de-identification and privacy. 

Despite its simplicity and ease of interpretablity, the EER is ill-suited as a measure of privacy.  Principally, this is because the EER reflects the perspectives of an evaluator and not those of a \emph{privacy adversary}.  While a framework to overcome these issues is proposed in~\cite{nautsch2020}, it addresses only one component of the anonymisation problem, namely that relating specifically to \emph{identity}; it does not reflect \emph{voice uniqueness}.  A solution to address both, i.e.\ a solution for the assessment of pseudonymisation, is the novel contribution in this paper.

We propose two pseudonymisation metrics for the assessment of de-identification and of voice uniqueness.  Speaker similarity matrices, upon which the two objective metrics are inspired, provide easily-interpretable visualisations of pseudonymisation behaviour and performance.  First, with a widely established privacy preservation terminology currently lacking, we provide definitions of de-identification and voice uniqueness.  We then present speaker similarity matrices and show how the two metrics are derived from them. Finally, we present the results of pseudonymisation experiments performed using the VoicePrivacy 2020 database and baseline systems.
